Unlocking the Secrets of Software Configuration Landscapes-Ruggedness, Accessibility, Escapability, and Transferability

Modern software systems are often highly configurable to tailor varied requirements from diverse stakeholders. Understanding the mapping between configurations and the desired performance attributes plays a fundamental role in advancing the controllability and tuning of the underlying system, yet has long been a dark hole of knowledge due to their black-box nature and the enormous combinatorial configuration space. In this paper, using $86$M evaluated configurations from three real-world systems on $32$ running workloads, we conducted one of its kind fitness landscape analysis (FLA) for configurable software systems. With comprehensive FLA methods, we for the first time show that: $i)$ the software configuration landscapes are fairly rugged, with numerous scattered local optima; $ii)$ nevertheless, the top local optima are highly accessible, featuring significantly larger basins of attraction; $iii)$ most inferior local optima are escapable with simple perturbations; $iv)$ landscapes of the same system with different workloads share structural similarities, which can be exploited to expedite heuristic search. Our results also provide valuable insights on the design of tailored meta-heuristics for configuration tuning; our FLA framework along with the collected data, build solid foundation for future research in this direction.

==> figs/tmp-pdfcrop-8878.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{6669745F646973747269627574696F6E2E706466}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{3}
\page 1 [32 204 1158 1172]
\csname @@end\endcsname
\end


==> makefile <==
FILE=main

all:	
	latex $(FILE)
	bibtex $(FILE)
	latex $(FILE)
	latex $(FILE)
	dvips -o $(FILE).ps $(FILE).dvi
	ps2pdf $(FILE).ps
	open $(FILE).pdf

clean:
	rm -f *.aux *.blg *.log *.bbl *.out *.bak *.synctex.gz *.synctex.gz\(busy\) *.tex~

cleanall: clean
	rm -f *.dvi $(FILE).ps $(FILE).pdf


==> sections/setup.tex <==
%!TeX root=main.tex

\section{Experimental Setup}
%\section{Case Studies}
\label{sec:setup}

This section introduces the setup of our empirical study, including the software systems under investigation, along with the configuration options and their corresponding performance metrics (\pref{tab:setup}). Due to the stringent page limit, more details are left in \textcolor{brightmaroon}{Appendix X} . 


